High Repetition-Rate Pulse Shaping of a Spectrally Broadened Yb Femtosecond Laser

We demonstrate compression and shaping of few cycle pulses from a high average power Ytterbium laser system. The pulses from a commercial 20 W, 100 kHz Yb laser system are spectrally broadened in two-stages using gas-filled, stretched hollow-core fibers and then compressed and shaped in an acousto-optic modulator-based pulse-shaper. The pulse-shaper allows for compression, characterization, and shaping all in one system, producing ~10 fs pulses with 50 uJ of energy

==> draft.tex <==
\section{Intro}
High average power ultrafast laser systems are increasingly in demand for many experiments which require high repetition rates for highly differential measurements, or ones which provide a very low yield per laser shot (e.g. coincidence measurements). While there are commercial Ytterbium laser systems available which can provide high average power with repetition rates of 100~kHz and greater, they typically produce pulses with durations greater than 100~fs. These long pulses are not suitable for many time-resolved spectroscopy or strong-field light matter experiments, which require few cycle pulses \BMK{}{to resolve the fastest molecular dynamics}. Here, we report on the spectral broadening and compression of 250~fs laser pulses from a 100~kHz 20~W commercial Ytterbium laser system (Light Conversion Pharos) using a dual stretched hollow-core fiber apparatus in conjunction with an acousto-optic modulator (AOM) based ultrafast optical pulse shaper \cite{fetterman1998ultrafast}. Our system is capable of producing arbitrarily shaped pulses as short as 10~fs, with energies between 30 and 50~$\mu$J, at repetition rates of up to 50~kHz.  

Shortening the duration of an ultrafast laser pulse can be broken into two stages: (1) broadening the pulse in the frequency domain, and (2) compression of the pulse in the time domain. Although there are many techniques to accomplish this \cite{nisoli1996generation, nagy2020generation, silletti2023dispersion}, spectral broadening is often achieved by propagating pulses through a gas-filled, hollow-core fiber (HCF), inducing self-phase modulation. Pulse compression is then usually achieved by applying negative group-delay dispersion (GDD) to the pulses with chirped mirrors. Few cycle pulses ($\sim$ 10~fs) have been generated at high average power by means of HCF-based spectral broadening and chirped-mirror-based pulse compression \cite{nagy2019generation}. However, using chirped mirrors and third-order dispersion-compensating material \cite{timmers2017generating} does not allow for programmable pulse shaping or direct compensation of higher order dispersion, which can be accomplished with an AOM based ultrafast pulse shaper \cite{jones2019dual,catanese2021acousto}. A further advantage of the direct dispersion control using an AOM based pulse shaper is that it can be used for pulse characterization, via techniques like dispersion scan (D-scan) \cite{miranda2012characterization} and collinear frequency resolved optical gating (CFROG) \cite{amat2004ultrashort}. 

Here, we demonstrate the production of an ultrabroadband spectrum with cascaded fibers and the ability to compress, control, and measure the pulses using an AOM-based 4f pulse-shaper. This work builds on our previous work \cite{catanese2021acousto}, but now uses a commercial Yb laser system, which enables us to perform pulse shaping at high repetition rates (50~kHz) and high pulse energies ($\sim$100 $\mu$J). We are able to compress 254 fs pulses from the output of the laser to pulses that are sub-10~fs, a compression factor of about 25. The combination of high average power and fine control of a broadened spectrum allows for highly differential time resolved spectroscopy measurements. 
  

\section{Apparatus}
\begin{figure}[h]
  \centering
  \includegraphics[width=1\textwidth]{Figures/Apparatusv4.png}
  \caption{\label{Apparatus}Experimental Apparatus. The pulses from the Yb laser are centered at about 1030 nm, with a 254~fs duration. They are focused into a 3~m long HCF filled with 3 bar of Ar and compressed with 4 bounces on chirped mirrors. They are then focused into a 2~m long HCF filled with 0.5~bar of Ar and sent into the AOM-based pulse shaper (the inset shows the mode of the beam exiting the pulse shaper). The compressed output of the pulse shaper is sent through a BBO crystal and into the spectrometer for characterization.}
\end{figure}
 
The schematic in Figure~\ref{Apparatus} shows the dual pulse-compression system and the subsequent measurement apparatus. In brief, each pulse-compression system consists of a spectral broadening component and a pulse compression component. Spectral broadening is achieved with Kerr-induced self-phase modulation by filling stretched hollow-core fibers with Argon \cite{nisoli1996generation,nagy}. Pulse-compression is done in two ways: after the first fiber, there are chirped mirrors, and after the second fiber, there is an AOM-based pulse-shaper. 

Pulses from a Yb laser (50~kHz repetition rate, 400~$\mu$J pulse energy, 20~W average power, 254~fs pulse duration, 1025 nm central wavelength) are focused to a beam waist of 144~$\mu$m and sent into the 3~m S-HCF. The inner diameter of the fiber is 450~$\mu$m, which corresponds to an optimal waist size of 144 $\mu$m in order to satisfy the mode matching condition \cite{abrams1972coupling}. The first fiber is glued onto mounts and stretched within a vacuum-sealable tube. The tube and enclosed fiber are filled with 3 bar of Ar. The efficiency of the first fiber is 73\%. The output of the fiber is collimated, and the spectrally broadened pulses are compressed in time with four bounces off of -500~fs$^2$ chirped mirrors. We estimate the pulse duration to be 35~fs after the first pulse-compression system based on calculations of the light matter interaction in the fiber, and the Fourier transform limit of the spectrum (Fig.~2). The exit of the first fiber is imaged onto the entrance of a second 2~m long S-HCF with the same mode matching condition as the first. In comparison to the first fiber, each end of the second fiber is fixed into a kinematic mount that is supported on a translation stage. So, the second fiber must be aligned to the laser, whilst the laser must be aligned into the first fiber. The second fiber is directly mated to the vacuum system and is filled with 0.5~bar of Ar. More details of the mounting method corresponding to the second fiber may be found in our previous paper \cite{catanese2021acousto}. The Fourier transform limit of the spectrum exiting the second fiber is 7~fs (Fig. 2), and the efficiency is 80\%. The output of the second fiber is collimated and the pulse is compressed using an AOM based pulse-shaper instead of chirped mirrors. 

\begin{figure}[h]
  \centering
  \includegraphics[width=.8\textwidth]{Figures/blueSpectraInset.PNG}
  \caption{\label{Spectra}Initial spectrum out of the laser centered about 1030~nm (light blue), spectrum out of the first fiber with a bandwidth of 80~nm tail-to-tail (medium blue), and spectrum out of the second fiber with a bandwidth of 400~nm tail-to-tail (dark blue) with an inset of the transform limit of the final spectrum.}
\end{figure}

\BMK{}{PULSE SHAPER PARAGRAPH 1: Optical components.}\\
\BMK{}{As shown in Fig. \ref{Apparatus} the pulse shaper is set-up in a 4f configuration with an AOM placed at the Fourier plane in the zero dispersion stretcher geometry. The shaper consists of two gold gratings...Repetition rate and other technical details.}

\BMK{}{PULSE SHAPER PARAGRAPH 2: How it works}\\
\BMK{}{First discuss the basic principle of the shaping: $E'(\omega) = M(\omega)E(\omega)$, where $E(\omega)$ is the input pulse, $E'(\omega)$ is the output shaped pulse, and $M(\omega)$ is the pulse shaper applied mask function. Then introduce the mapping the mapping of acoustic time to optical frequency $t\rightarrow \omega$. Next, connect the mask with the system with the following equation:}
\begin{equation}
    V(t)=|M(\omega(t))|\cos(2\pi f_{\text{rf}}t+\arg(M(\omega(t))))
\end{equation}
\BMK{}{This equation describes the acoustic wave that is in the crystal. Finally, discuss how the non-linear mapping introduces an optical phase that changes with AOM orientation and how that can be used to compress the pulse}

The pulse-shaper is a 4f system \BMK{following earlier}{as discussed in earlier work Ref.} \cite{jones2019dual, catanese2021acousto}, but optimized for a near-IR, high average power laser. Pulses with 10 W average power and a bandwidth of 450 nm tail-to-tail are the input of the pulse shaper, so a gold coated ruled diffraction grating blazed for 1025 nm is used. The first order diffracted beam is propagated to a 50 cm, gold coated curved mirror and focused into a TeO$_2$ AOM, which is placed in the Fourier plane of the zero dispersion stretcher geometry. The grating and focusing mirror map the optical frequencies of the laser pulse to position in the AOM. Given the relatively slow velocity of the acoustic wave in the crystal compared with the speed of light, the acoustic wave \BMK{in the AOM} is essentially frozen as the laser pulse propagates \BMK{}{orthgonally }through the \BMK{AOM}{crystal}.  Thus, the optical frequencies \BMK{are}{can be} mapped to time in the acoustic wave.  While this mapping is roughly linear with optical wavelength for small diffraction angles ($\sin(\theta)\sim \theta$), the mapping of optical frequency to acoustic time is highly nonlinear given the inverse relationship between frequency and wavelength. This non-linearity leads to higher order dispersion \cite{jones2019dual} \BMK{}{when programming the constant acoustic wave for the laser to diffract off of}. \BMK{}{However, }based on the placement of the AOM \cite{catanese2021acousto}, the \BMK{programmable dispersion can be}{sign of this dispersion can be controlled and} utilized to compensate for positive dispersion from optics in the beam path. Here, the transducer of the AOM is on the red side of the optical spectrum and the +1 diffraction order is used, and the diffraction efficiency is 55\%. \BMK{We are limited in repetition rate from the laser’s 100 kHz maximum to 50 kHz because the time for the acoustic wave to fill the crystal is 10 $\mu$s, and the entire AOM aperture is filled with bandwidth.}{The maximum repetition rate is limited by the transit time of the acoustic wave through the active portion of the crystal. As we utilize the entire crystal to shape the optical bandwidth this corresponds to 10 $\mu$s or a maximum repetition rate of 100 kHz. However, this version of the laser system has half the output energy at 100 kHz as it does at 50 kHz limiting us to shaping at 50 kHz for the shaping of experimentally relevant pulses.} The shaped pulses exit the pulse shaper in a symmetrically equivalent way to the input pulses. The efficiency of the 4f AOM-based pulse shaper is 25\%. 

\comment{To measure the pulse duration, D-scans and CFROGs were taken. Pulses are sent through a 10 $\mu$m thick BBO crystal and the resulting SHG spectrum is recorded. For D-scans, GDD was scanned through at specified third order (TOD) and fourth order dispersion (FOD) by programming these values to the pulse shaper. We note that it is useful to start with a long, coarse GDD scan at 0 fs$^3$ TOD and 0 fs$^4$ FOD and iterate the higher orders based on the shape of the D-scan. Similarly, for CFROGs, the delay between pulses is programmed and scanned through by the pulse shaper. }

\BMK{}{Dispersion is often described in terms of a Taylor series expansion. Thus, we utilize the same formulation for the pulse shapers dispersion control and write the mask:}
\begin{equation}
    M(\omega) = \exp\bigg(i\frac{\text{GDD}}{2}(\omega-\omega_0)^2 + i\frac{\text{TOD}}{6}(\omega-\omega_0)^3 + i\frac{\text{FOD}}{24}(\omega-\omega_0)^4\bigg)
    \label{eq:compression}
\end{equation}
\BMK{}{where $\omega_0$ is the central frequency of the expansion, GDD is the group delay dispersion, TOD is the third order dispersion, and FOD is the fourth order dispersion. Two techniques were used to measure the pulse duration: D-scans and CFROGs. The pulses are sent through a 10 $\mu$m thick BBO crystal and the resulting SHG spectrum is recorded. For D-scans, GDD was scanned through at a specified third order (TOD) and fourth order dispersion (FOD) by programming these values to the pulse shaper. We note that it is useful to start with a long, coarse GDD scan at 0 fs$^3$ TOD and 0 fs$^4$ FOD and iterate the higher orders based on the shape of the D-scan. }

\BMK{}{Similarly, for CFROGs, the dispersion (GDD, TOD, and FOD) are fixed and the delay between pulses is programmed and scanned through by the pulse shaper utilizing the mask:}
\begin{equation}
    M(\omega) = 1+R\exp\big(i(\omega-\omega_L)\tau+i\phi_L\big)
    \label{eq:CFROG}
\end{equation}
\BMK{}{where $R$ is the relative pulse amplitude, $\omega_L$ is the locking frequency (frequency at which constructive interference occurs independent of delay), $\tau$ is the pulse delay, and $\phi_L$ is the relative pulse phase. As CFROGs use a collinear geometry they are easier to set-up and remove the potential for temporal smearing compared to typical FROGs, and while normally the scan step would require sampling of the carrier an appropriate choice of $\omega_L$ softens this requirement such that one only needs a step size to sample the envelope.}

\section{Apparatus Discussion}
Multiple avenues of pulse compression were attempted to achieve sub-10 fs pulses. We originally tried to compress the 254 fs pulses out of the laser with a single S-HCF, filled with molecular gas, and the AOM-based pulse-shaper. We filled the fibers with molecular gas because spectral broadening can be enhanced by the rotational Raman process \cite{fan2020high}. The most promising gas seemed to be N$_2$O based on the Fourier transform limit of the spectrum out of the fiber. However, at average powers of 10 W or greater, the molecular gas absorbed too much energy from the laser as a result of rotational heating, dramatically decreasing the throughput efficiency and damaging the entrance to the optical fiber. Thus, we made use of atomic gases, for which the nonlinear process is strictly parametric, with no heating of the gas. This however, required two fibers in order to produce the desired bandwidth and final pulse duration.  

High average power through the pulse shaper also needed to be considered.  Too high a peak intensity in the AOM can lead to self focusing and self phase modulation, and too high an average power on the diffraction gratings can lead to mode distortions.  While increasing the mode size into the pulse shaper mitigates the mode distortions due to nonuniform thermal expansion of the gratings, it leads to a tighter focus in the AOM, which can lead to both self focusing and damage. Therefore, we had to strike a balance between these two requirements, and used a mode size of \BMK{}{XXX} mm FWHM going into the pulse shaper.  We tried two different pairs of gratings - one with 300~lines/mm, and another with 200~lines/mm.  Both were gold coated ruled diffraction gratings blazed for operation at about 1000~nm.  They both consist of a glass substrate with an epoxy that was used to produce a replica grating from a ruled master, coated with a thin layer of chromium and then gold. Combined with the 500~mm focal length mirrors, the dispersed spectrum with the 300~lines/mm grating was too large for the aperture of the AOM, limiting the spectrum and compression to 20~fs. At average powers over 10~W, these gratings in the pulse shaper became deformed by the thermal load from the laser and this decreased the efficiency of the pulse shaper to 20\%, but the mode and power were stable. For the gratings with a groove density of 200~lines/mm, we were able to compress the pulses to $\sim$10~fs, but these gratings provided lower efficiency and were damaged at average powers over 10~W.  We considered changing the curved mirrors to ones with a shorter focal length to fit more of the bandwidth on the AOM, but this would also increase the vertical focus of the beam. Currently, we are in the process of procuring a 150~lines/mm grating $\ge$1 in$^2$ on an appropriate substrate to minimize thermal effects. These will also allow us to fit the entire bandwidth onto the AOM aperture. 

\begin{figure}[H]
  \centering
  \includegraphics[width=.7\textwidth]{Figures/OverallOutputv2.png}
  \caption{\label{Spectra} Overall pulse energy out of the system after the pulse shaper with two different gratings: 300 lines/mm (blue) and 200 lines/mm (red).}
\end{figure}

\section{Results}
With this system, we are able to compress the 254~fs pulses out of the laser down to 11~fs pulses. One of the strengths of the AOM-based pulse shaper is that it allows for different types of pulse characterization. By writing a mask on the phase of the acoustic wave, we can scan through the second order dispersion (GDD) and adjust the third (TOD) and fourth (FOD) order dispersion accordingly, \BMK{}{ie Eq. \ref{eq:compression}}. For CFROGs, we can utilize the same phase mask and scan through the delay between two pulses \BMK{}{(product of Eqs. \ref{eq:compression} and \ref{eq:CFROG}}. Figure 4 shows a D-scan and CFROG that reconstruct to 11.0 fs and 11.5 fs, respectively. To obtain the D-scan, the GDD was scanned from 6200 to 8000 fs$^2$, and the applied TOD and FOD were -23700 fs$^3$ and 55000 fs$^4$. (Include GDD table things.)
\input{gvdtable}
With the acquired GDD, TOD, and FOD, we then scanned the delay between a pair of pulses. The reconstructed duration for both types of pulse characterization agree within 0.5 fs. The Fourier transform limited duration calculated with the bandwidth measured after the pulse shaper was 7.8 fs. \BMK{}{$\omega_L=XXX$rad/fs and $\phi_L=0$}

\begin{figure}[H]
    \centering
    \includegraphics[width = 0.9\textwidth]{Figures/bluepulseCharacterization.PNG}
    \caption{Top panel: an AOM-based pulse-shaper D-scan and its corresponding, reconstructed pulse duration (11.0 fs) and phase. Bottom panel: an AOM-based pulse-shaper CFROG and its corresponding, reconstructed pulse duration (11.5 fs) and phase.}
\end{figure}

\BMK{An advantage of using the pulse shaper is that the delay between pulse pairs can be fixed, which eliminates the challenges of setting up an interferometer to create pairs of pulses. At such short pulse durations, this common FROG setup may introduce temporal smearing, which artificially increases the recorded pulse duration.}{} Figure 5 is a testament to the ability of the pulse shaper. It shows a CFROG characterization of two pulses that were delayed by 50 fs, but the two pulses were $\pi$ out of phase with each other on the top panel and in phase on the bottom panel. This phase difference can be seen nicely in the intensity plots to the right of the CFROGs. At 50 fs in the CFROG delay, the pulses destructively interfere when they are out of phase and constructively interfere when they are in phase. \BMK{}{I would reference the masks discussed earlier. Potentially, it might make sense to explicitly write out the mask that was used here as it has not been discussed before in any of our work.}

\begin{figure}[H]
    \centering
    \includegraphics[width = 1\textwidth]{Figures/blueDoublePulse.PNG}
    \caption{CFROG characterizations of double pulses where the pulses in the top panel were $\pi$ out of phase and the pulses in the bottom panel were in phase. The plots to the right of the CFROGs are the integrated intensity of the CFROGs over wavelength.}
    \label{fig:10kHzCharSummary}
\end{figure}

\section{Conclusion}
We have demonstrated the ability to achieve a high compression ratio of pulses with high pulse energy and repetition rate. The pulses can be shaped in phase and amplitude with the AOM-based pulse shaper, and pulse pairs can be created with fixed time delays. This allows us to both create ultrafast pulses, on the order of 10 fs, and characterize them with the same device. Currently, we are limited by the efficiency and groove density of our diffraction gratings, but have shown the capability of 1 in$^2$ gratings to handle high average power and low groove density gratings to handle large bandwidths. The generation of intense, ultrafast pulses with arbitrary delays between pulse pairs will allow for pump probe measurements of molecular dynamics \cite{tagliamonti2017time}. *I'm not sure of the technical vocab about why the higher pulse energies are better, compared to the previous setup.*

%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{Figures/Characterization_v1.png}
%    \caption{Caption}
%    \label{fig:enter-label}
%\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width = 0.9\textwidth]{Figures/pulseCharacterizationD26C1.png}
    \caption{Top panel: an AOM-based pulse-shaper D-scan and its corresponding, reconstructed pulse duration (10.5 fs) and phase. Bottom panel: an AOM-based pulse-shaper CFROG and its corresponding, reconstructed pulse duration (14 fs) and phase.}
\end{figure}


\section{Figures}
\begin{itemize}
\item Figure 1 apparatus with Pharos with specs on what comes out of that box, then two fibers with chirped mirrors between fibers plus AOM pulse shaper with Moku after second fiber and show FROG/Dscan apparatus - super simple
\item Pulse compression figure - Dscan plus spectrum plus CFROG plus phaselocked CFROG for comparison?
\item Details figures - spectrum out of first fiber and second fiber, pulse shaper performance vs rep rate, blah blah
\end{itemize}
\section{Highlights}
\begin{itemize}
\item High average power compressed, shaped, and characterized with AOM pulse shaper.
\item phase locked CFROG - check Ogilvie work (Brian knows about)
\item Dscan of any duration
\item Julia's spectrometer for near IR using BBO crystal
\item note that Dscan is very good at characterizing spectral phase and correcting it but not good for pre/post pulse characterization, whereas CFROG is complement for this which is good for pre/post pulse structures but not good for compression or characterizing spectral phase as easily.
\item also mention things that we tried and didn't work so well, or difficulties with the project in general
\end{itemize}
\section*{}

% The generation of high energy few-cycle laser pulses are an enabling technology for strong field science and time-resolved measurements. In particular these sources have proved instrumental in both strong field ionization and high harmonic generation,
% and therefore serve as a cornerstone of attosecond science [ref]. However, despite the production of these pulses now be routine, the precise manipulation of the often octave spanning bandwidth and generation of arbitrary fields is challenging. One methodology that has allows exquisite control over laser fields is pulse shaping, which has had limited application for such broadband pulses. This is particularly egregious given the developments in multidimensional, in particular 2D, spectroscopy exploiting pulse shapers, where these octave spanning pulses could help advanced our understanding of processes like protein folding and solvation as well as the workings of light harvesting complexes and the photosynthetic reaction centers (cite).

% Here we demonstrate spectral broadening of a commercial high average power femtosecond ytterbium (Yb) laser (Light Conversion Pharos ) as well as the manipulation and direct compression of the resultant pulses using an acousto-optic modulator(AOM) based pulse shaper. This work builds our recent demonstration of manipulating and compressing of octave spanning few-cycle laser pulses using this approach (cite) and extends this to the case of high repetition rate and high average power laser pulses. 

% A home built stretched hollow-core fiber (HCF) apparatus, filled with XX molecules, is used to significantly extend the spectral content of our femtosecond laser system (cite). An overview of the experimental setup is presented in Fig.~\ref{Setup_spectra} alongside the pressure dependence of the output spectra from the HCF apparatus and the associated Fourier transform limited pulse duration based of these spectra. By exploiting a large core diameter, alongside the HCF stretching (cite), we achieve excellent throughput (XX\%) for this system. 

% \begin{figure}[htbp]
%   \centering
%   %\includegraphics[width=8.3cm]{OT10000F1}
% \caption{\label{Setup_spectra}(a) Experimental setup and (b) output spectra.}
% \end{figure}

% Traditionally the output of spectral broadening schemes, such as gas-filled HCFs, has been compressed via chirped mirrors and the production of intense few-cycle laser pulses for strong-field science and attosecond pulse generation is now routine. Instead of chirped mirrors we compress the output of our HCF with an AOM pulse shaper (cite), which provides several key advantages, including direct compensation of high order dispersion, built in pulse characterization (collinear programmable and D scan measurements), and the ability to produce arbitrary pulse shapes with pulses as short as two optical cycles.  The employed grating (xxxxx), curved mirror and AOM (XXXX) 4-f setup has XX\% throughput at a repetition rate of XX~kHz. The resulting in an pulse energy, in excess of XX~$\mu$J, is suitable for a variety of multidimensional spectroscopy and strong-field science experiments on isolated atoms and molecules. 

% Beyond compression and manipulation the pulse shaper provides another key advantage that pulses can be characterized using shaper assisted versions of the dispersion scan (D-scan) and frequency resolved optical gating (FROG) (cite). Shown in Fig.~\ref{FROG} are collinear (C) FROG traces and the associated reconstruction of our output pulses for an employed HCF pressure of XX~bar of YY. Highlighted is the excellent compression achieved by our approach where pulses were able to be compress the pulses to within $\approx$X~fs of the YY~fs transform limit. 

% \begin{figure}[htbp]
%   \centering
%   %\includegraphics[width=8.3cm]{OT10000F1}
% \caption{\label{FROG}FROG}
% \end{figure}

% We demonstrate compression, measurement and control of broadband pulses from a home built stretched HCF apparatus using a programmable AOM-based 4f pulse-shaper. Unlike previous results, we demonstrate the ability to do pulse shaping at high repetition rates (XX~kHz) and high pulse energies (YY~$\mu$J). Measurements of the pulse duration obtained by the pulse-shaper CFROG showcased compression down to XX~fs. The ability to generate intense pulses with the pulse-shaper enables pump probe measurements with phase locked pulses and arbitrary (delay dependent) relative amplitudes, which will be an important tool for strong-field coherent control experiments at high repetition rates. Future work to extend the current methodology to high repetition rate octave spanning pulses is underway. 

% MAYBE MENTION HOW OTHER PULSE SHAPING APPROACHES WOULD RUN INTO DIFFICULTIES AND HOW WHAT WE ARE DOING EXPLOITS THE LIMITS OF WHAT AOMS CAN DO.

% This work was funded by the Linac Coherent Light Source, SLAC National Accelerator Laboratory, which is supported by the U.S. Department of Energy, Office of Science, Office of Basic Energy Sciences, under Contract No. DE-AC02-76SF00515 and XXX. 


%\subsection{Required Elements}
%All PDF submissions must contain the following items in order to be published:

%\begin{enumerate}
%\item Complete title
%\item Complete listing of all authors and their affiliations
%\item Self-contained abstract (indexers such as Google Scholar will not index papers that do not contain abstracts)
%\item Appropriate copyright statement following the abstract. By default, the copyright statement will appear as \number\year \hskip.05in The Author(s). If needed, the default statement can be suppressed by use of the \verb+{abstract*}+ environment.
%\item Permission and attribution for any trademarked or copyright images. Note that images of people or images owned or trademarked by other entities (including well-known logo's or cartoon characters for example) will also require official written permission.
%\item Two-page limit unless designated otherwise on conference website
%\end{enumerate}

%\subsection{Typographical Style}
%Margins and type size will be set by the Optica \LaTeX{}
%commands for title, author names and addresses, abstract,
%references, captions, and so on. The \texttt{opticameet3.sty} package
%references \texttt{mathptmx.sty} for Times text and math fonts.
%Authors who require Computer Modern font may modify the style file
%or, preferably, invoke the package \texttt{ae.sty} or similar for
%optimum output with Computer Modern.

%\subsection{Author Names and Affiliations}
%Author names should be given in full with first initials spelled out to assist with indexing.
%Affiliations should follow the format division, organization, and address---and complete postal information should be given.
%Abbreviations should not be used. United States addresses should end
%with ``, USA.''

%\subsection{Abstract} The abstract
%should be limited to no more than 35 words. It should be an
%explicit summary of the paper that states the problem, the methods
%used, and the major results and conclusions. If another publication author is referenced in the abstract, abbreviated information
%(e.g., journal, volume number, first page, year) must be
%given in the abstract itself, without a reference number. (The item referenced in the abstract should be the first
%cited reference  in the body.)

%\subsection{Notation}
%\subsubsection{General Notation}
%Notation must be
%legible, clear, compact, and consistent with standard usage. In
%general, acronyms should be defined at first use.


%\subsubsection{Math Notation}
%Equations should use standard \LaTeX{} or AMS\LaTeX{} commands (sample from Krishnan %\textit{et al.} \cite{krishnan00}).

%\begin{eqnarray}
%\bar\varepsilon &=& \frac{\int_0?\infty\varepsilon
%\exp(-\beta\varepsilon)\,{\rm d}\varepsilon}{\int_0?\infty
%\exp(-\beta\varepsilon)\,{\rm d}\varepsilon}\nonumber\\
%&=& -\frac{{\rm d}}{{\rm d}\beta}\log\Biggl[\int_0?\infty\exp
%(-\beta\varepsilon)\,{\rm d}\varepsilon\Biggr]=\frac1\beta=kT.
%\end{eqnarray}

%\section{Tables and Figures}
%Figures and illustrations should be incorporated directly into the
%manuscript, and the size of a figure should be commensurate with the amount
%and value of the information conveyed by the figure.

%\begin{table}[htb]
% \centering \caption{Sample Table}
%\begin{tabular}{ccc}
%    \hline
%    One & Two & Three \\
%    \hline
%    Eins & Zwei & Drei \\
%    Un & Deux & Trois \\
%    Jeden & Dv\v{e} & T\v{r}i \\
%    \hline
%   \end{tabular}
%    \end{table}

%No more than three figures should generally be included in the paper. Place figures as close as possible to where they
%are mentioned in the text. No part of a figure should extend beyond text width, and text should not wrap around figures. Please provide permission and attribution for any trademarked or copyright images.

%References should be cited with the \verb+\cite{}+ command.
%Bracketed citation style, as opposed to superscript, is preferred
%\cite{krishnan00,vantrigt97,masters93,shoop97,kalman76,craig96,steup96}.
%The \texttt{opticameet3.sty} style file references \texttt{cite.sty}. Comprehensive journal abbreviations are available on the Crossref web site:
%\href{http://www.crossref.org/titleList/}{http://www.crossref.org/titleList/}.

%\begin{thebibliography}{99}
%\bibliographystyle{unsrt}

%\bibitem{krishnan00} E. Krishnan, A. M. Shan, T. Rishi, L. A. Ajith, C. V.
%Radhakrishnan, \textit{On-line Tutorial on \LaTeX{}},
%``Mathematics'' (Indian \TeX{} Users Group, 2000), \\
%\url{http://www.tug.org/tutorials/tugindia/chap11-scr.pdf}.

%\bibitem{vantrigt97} C. van Trigt, ``Visual system-response functions and %estimating reflectance,''
%J. Opt. Soc. Am. A \textbf{14}, 741--755 (1997).

%\bibitem{masters93} T. Masters, \emph{Practical Neural Network Recipes in C++} (Academic, 1993).

%\bibitem{shoop97} B. L. Shoop, A. H. Sayles, and D. M. Litynski, ``New devices for optoelectronics: smart pixels,''
%in \emph{Handbook of Fiber Optic Data Communications},
%C. DeCusatis, D. Clement, E. Maass, and R. Lasky, eds. (Academic, 1997), pp. 705--758.

%\bibitem{kalman76} R. E. Kalman,``Algebraic aspects of the generalized inverse of a rectangular matrix,'' in
%\emph{Proceedings of Advanced Seminar on Generalized Inverse and Applications}, M. Z. Nashed, ed. (Academic, 1976), pp. 111--124.

%\bibitem{craig96} R. Craig and B. Gignac, ``High-power 980-nm pump lasers,''
%in \emph{Optical Fiber Communication Conference}, Vol. 2 of 1996 OSA Technical Digest Series (Optical Society of America, 1996), paper ThG1.

%\bibitem{steup96} D. Steup and J. Weinzierl, ``Resonant THz-meshes,''
%presented at the Fourth International Workshop on THz Electronics, Erlangen-Tennenlohe, Germany, 5--6 Sept. 1996.

%\end{thebibliography}

==> finalGVDtable.tex <==
\begin{table}[H]
\centering
\begin{tabular}{cccc} \toprule
 Dispersive Elements & GDD (fs$^2$) & TOD (fs$^3$) & FOD (fs$^4$) \\ \midrule %[0.5ex]
 Lens  & 68 & 123 & -136 \\
 %Window  & 61 & 121 & -141 \\
 %$\frac{1}{2}$ Waveplate  & 150 & 326 & -400 \\
 Air        & 65  & 9 & - \\
 AOM TeO$_2$  & 3618 & 2583 & 1172 \\
 Ar Broadening & 250 & - & - \\ 
 Nonlinear Mapping & -10624 & 16350 & -24201 \\ \midrule
 Sum of Elements & -6623 & 19065 & -23165 \\
 Applied Phase Mask & 7166 & -23700 & 55000 \\ \midrule\midrule
 Sum + Mask & 543 & -4635 & 31835 \\ \bottomrule
\end{tabular}
\caption{Table comparing the sum of the applied dispersion and dispersion accumulated along the table. To have the shortest compressed pulse, we expect the sum of the elements and the applied mask to cancel each other out.}
\label{tab:dtable}
\end{table}

==> gvdtable.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cccc} \toprule
 Dispersive Elements & GVD (fs$^2$) & TOD (fs$^3$) & FOD (fs$^4$) \\ \midrule %[0.5ex]
 Lens  & 68 & 123 & -136 \\
 %Window  & 61 & 121 & -141 \\
 %$\frac{1}{2}$ Waveplate  & 150 & 326 & -400 \\
 Air        & 65  & 9 & - \\
 AOM TeO$_2$  & 3618 & 2583 & 1172 \\
 Ar Broadening & 250 & - & - \\
 %\footnote{The GVD of Fiber 1 broadening was estimated from calculations of dispersion simulations conducted by Ruaridh Forbes at SLAC. This estimate is also supported by simulations of Fiber 2 broadening with an incoming pulse at the TL of the input spectrum.} &   &   \\ \hline
 Applied Phase Mask & 7166 & -23700 & 55000 \\ \midrule
 Sum of Elements & 11167 & -20985 & 56036 \\
 Nonlinear Mapping & -11813 & 35671 & -92074 \\ \midrule\midrule
 Sum + Mapping & -646 & 14686 & -36038 \\ \bottomrule
\end{tabular}
\caption{Third order calib. Table of the dispersion along the path of the pulse.}
\label{tab:dtable}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{cccc} \toprule
 Dispersive Elements & GVD (fs$^2$) & TOD (fs$^3$) & FOD (fs$^4$) \\ \midrule %[0.5ex]
 Lens  & 68 & 123 & -136 \\
 %Window  & 61 & 121 & -141 \\
 %$\frac{1}{2}$ Waveplate  & 150 & 326 & -400 \\
 Air        & 65  & 9 & - \\
 AOM TeO$_2$  & 3618 & 2583 & 1172 \\
 Ar Broadening & 250 & - & - \\
 %\footnote{The GVD of Fiber 1 broadening was estimated from calculations of dispersion simulations conducted by Ruaridh Forbes at SLAC. This estimate is also supported by simulations of Fiber 2 broadening with an incoming pulse at the TL of the input spectrum.} &   &   \\ \hline
 Applied Phase Mask & 7166 & -23700 & 55000 \\ \midrule
 Sum of Elements & 11167 & -20985 & 56036 \\
 Nonlinear Mapping & -9898 & 19056 & -52217 \\ \midrule\midrule
 Sum + Mapping & 1269 & -1929 & 3819 \\ \bottomrule
\end{tabular}
\caption{Fourth order calib. Table of the dispersion along the path of the pulse.}
\label{tab:dtable}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{cccc} \toprule
 Dispersive Elements & GVD (fs$^2$) & TOD (fs$^3$) & FOD (fs$^4$) \\ \midrule %[0.5ex]
 Lens  & 68 & 123 & -136 \\
 %Window  & 61 & 121 & -141 \\
 %$\frac{1}{2}$ Waveplate  & 150 & 326 & -400 \\
 Air        & 65  & 9 & - \\
 AOM TeO$_2$  & 3618 & 2583 & 1172 \\
 Ar Broadening & 250 & - & - \\
 %\footnote{The GVD of Fiber 1 broadening was estimated from calculations of dispersion simulations conducted by Ruaridh Forbes at SLAC. This estimate is also supported by simulations of Fiber 2 broadening with an incoming pulse at the TL of the input spectrum.} &   &   \\ \hline
 Applied Phase Mask & 7166 & -23700 & 55000 \\ \midrule
 Sum of Elements & 11167 & -20985 & 56036 \\
 Nonlinear Mapping & -10624 & 16350 & -24201 \\ \midrule\midrule
 Sum + Mapping & 543 & -4635 & 31835 \\ \bottomrule
\end{tabular}
\caption{Inverse function calibration. Table of the dispersion along the path of the pulse.}
\label{tab:dtable}
\end{table}

==> snlo.tex <==
for 1030 (o) + 1030 (o) = 515 (e)
Mix accpt bwXL = 1053.07 GHz*cm

for 20 um bbo crystal -> 
bw = 10/20 * 1053.07 THz
500 THz
or 
